Embodiment-Agnostic Navigation Policy Trained with Visual Demonstrations

Learning to navigate in unstructured environments is a challenging task for robots. While reinforcement learning can be effective, it often requires extensive data collection and can pose risk. Learning from expert demonstrations, on the other hand, offers a more efficient approach. However, many existing methods rely on specific robot embodiments, pre-specified target images and require large datasets. We propose the Visual Demonstration-based Embodiment-agnostic Navigation (ViDEN) framework, a novel framework that leverages visual demonstrations to train embodiment-agnostic navigation policies. ViDEN utilizes depth images to reduce input dimensionality and relies on relative target positions, making it more adaptable to diverse environments. By training a diffusion-based policy on task-centric and embodiment-agnostic demonstrations, ViDEN can generate collision-free and adaptive trajectories in real-time. Our experiments on human reaching and tracking demonstrate that ViDEN outperforms existing methods, requiring a small amount of data and achieving superior performance in various indoor and outdoor navigation scenarios. Project website: https://nimicurtis.github.io/ViDEN/.

==> related.tex <==



\subsection{Traditional Navigation and Planning}

Traditional navigation methods provide robust frameworks for collision-free, goal-directed movement, relying on perception, localization, and path planning. Perception uses sensor inputs like LIDAR or depth cameras to construct environmental maps, such as occupancy grids \cite{elfes1989using} or voxel-based representations \cite{hornung2013octomap}. Localization techniques like SLAM \cite{cadena2016past} estimate the robot's position, while planning algorithms, such as A* \cite{hart1968formal} and RRT \cite{lavalle1998rapidly}, compute paths while accounting for obstacles and dynamics.
However, these methods depend on detailed maps, which are often impractical in dynamic settings and require a significant amount of effort to tune parameters for these methods to adapt to a wide range of scenarios\cite{thrun2005probabilistic}, and their computational complexity grows with environmental size \cite{karaman2011sampling}. Moreover, reliance on precise sensors limits their adaptability to noisy or low-cost platforms \cite{cadena2016past}.




\subsection{Learning based}

\begin{itemize}
    \item \cite{wang2023mimicplay} MimicPlay: Example of human play data collection, showcasing how easy and efficient it is to capture diverse task-centric data without the need for robot hardware.
    \item \cite{chi2024universal} UMI: Demonstrates universal manipulation with imitation learning, focusing on generalizable policies.
    \item \cite{ha2024umilegsmakingmanipulation} UmiOnLegs: Explores diffusion-based imitation learning applied to quadruped robots for advanced manipulation tasks.
    \item \cite{sridhar2023nomadgoalmaskeddiffusion} NoMaD: Builds upon ViNT with diffusion-based navigation and exploration, introducing goal masking for multi-modal policies.
    \item \cite{shah2023vintfoundationmodelvisual} ViNT: The foundation model for robot navigation, employing transformer-based policies for versatile and scalable navigation tasks.
    \item \cite{shah2023gnmgeneralnavigationmodel} GNM: The predecessor of ViNT, focusing on generalizing navigation across diverse robots and environments.
    \item \cite{yu2024ldp} LDP: A method for robot local navigation with diffusion models, leveraging local cost maps, goal states, and precomputed global paths.
    \item \cite{hirose2024lelan} LeLAN: Proposes learning to navigate from online videos, enabling robots to learn navigation behaviors directly from human video demonstrations.
    \item \cite{reuss2023} Goal-conditioned imitation learning with score-based diffusion policies: This work extends diffusion models to goal-conditioned tasks, providing insights into robust trajectory prediction under multi-modal distributions.
    \item \cite{ding2020} Goal-conditioned imitation learning: Explores imitation learning frameworks for achieving specified goals, focusing on efficient policy training under sparse rewards.
    \item \cite{andrychowicz2018hindsightexperiencereplay} Hindsight Experience Replay (HER): Introduces a data augmentation technique to improve learning in sparse reward environments by reinterpreting failed attempts as successful outcomes for alternative goals.
\end{itemize}

\subsection{Learning-Based Navigation}

Recent advancements address the limitations of traditional methods by integrating machine learning and data-driven approaches. Learning-based frameworks infer navigation policies directly from sensor data, bypassing the need for explicit maps and enabling robust operation in dynamic environments \cite{}. However, these approaches often demand extensive data collection and computational resources, motivating hybrid techniques that blend traditional planning with learning-based enhancements.

Numerous studies have proposed innovative strategies to advance learning-based imitation. MimicPlay \cite{wang2023mimicplay} utilizes human play data to efficiently capture diverse trajectories with minimal effort. Umi \cite{chi2024universal} introduces a custom handheld gripper to simplify data collection and bridge gaps in manipulation tasks. Additionally, in \cite{ha2024umilegsmakingmanipulation} they applied diffusion-based imitation learning for quadruped robot manipulation. NoMad \cite{sridhar2023nomadgoalmaskeddiffusion} expands this diffusion-based approach to navigation and exploration tasks, building on ViNT \cite{shah2023vintfoundationmodelvisual}, a foundational robot navigation model derived from the General Navigation Model (GNM) \cite{shah2023gnmgeneralnavigationmodel}. Local Diffusion Policies (LDP) \cite{yu2024ldp} further leverage diffusion models for navigation by utilizing local cost maps, global paths, and predefined goals. Meanwhile, Hirose et al. \cite{hirose2024lelan} propose a novel framework for learning navigation policies directly from online videos, reducing the need for explicitly curated robotic datasets.


